Does RoBERTa Perform Better than BERT in Continual Learning: An Attention Sink Perspective

Continual learning (CL) aims to train models that can sequentially learn new tasks without forgetting previous tasks' knowledge. Although previous works observed that pre-training can benefit CL, it remains unclear whether a pre-trained model with higher downstream capacity also performs better in CL. In this paper, we observe that pre-trained models may allocate high attention scores to some 'sink' tokens, such as [SEP] tokens, which are ubiquitous across various tasks. Such attention sinks may lead to models' over-smoothing in single-task learning and interference in sequential tasks' learning, which may compromise the models' CL performance despite their high pre-trained capabilities. To reduce these effects, we propose a pre-scaling mechanism that encourages attention diversity across all tokens. Specifically, it first scales the task's attention to the non-sink tokens in a probing stage, and then fine-tunes the model with scaling. Experiments show that pre-scaling yields substantial improvements in CL without experience replay, or progressively storing parameters from previous tasks.

==> analysis_yifan.tex <==
\section{Attention Sink and Interference in Continual Learning} \label{sec:interference_sink}
In this section, we show how attention sinks can cause interference in CL settings. We first define the cross-task interference with gradients. Then we conduct a case study to show that attention sinks characterized in Section \ref{sec:single_task_sink} can cause unnecessary interference when learning across tasks. Finally, we discuss a transfer vs. interference trade-off which suggests that attention sinks are important for model capacity and transfer learning. To reduce the interference while preserving model capacity, we propose a pre-scaling mechanism in Section 5.
%focus on a CL setting where we sequentially learn a model on Task 1 and Task 2. 
%Similar to Eq. (\ref{eqn:dist_define}), we define the cross-task representation distance below.

\subsection{{Interference in Continual Learning}}
We study the following CL problem: A model continually learns a sequence of tasks, with the previous tasks' data inaccessible when learning new tasks. The model has different class vectors for classes in different tasks, while other parameters are shared. Each  task $i$ consists of data $\mathcal{D}_i = ({\bf{X}}_i, y_i)$ where ${\bf{X}}_i$ is the input data at task $i$, and $y_i \in \mathbb{R}$ is its target output. 

When learning task $j$ after task $i$, the cross-task interference on the shared parameter $\theta$ can be defined as the dot product between its (vectorized) gradients on two tasks' losses \citep{riemer2018learning}: 
\begin{align}
    I(\theta; i, j) = \nabla_\theta L({\bf{X}}_i, y_i)\nabla_\theta L({\bf{X}}_j, y_j) %\nonumber
    \label{eqn:cross-task-interference}
\end{align}
where $\cdot$ is the dot product operator on the flattened gradients. The interference that leads to forgetting happens when $I(\theta; i, j) < 0$, while the knowledge transfer may happen if $I(\theta; i, j) > 0$. For tasks that do not have knowledge transfer, the interference is expected to be 0.

\subsection{{Case Study: Attention Sink Can Cause Unnecessary Interference Between Tasks}}
%We use a case study to show how attention sinks can propagate unexpected interference between otherwise orthogonal tasks.
%The study is based on the attention sink phenomenon characterized in Section \ref{sec:single_task_sink}: (1). models allocate high attention to sink tokens with small deviations; (2). sink tokens are usually common tokens shared across different tasks.  

%\paragraph{Data.} %\nb{State english first then specific notation.} 
Consider two unrelated tasks in a CL setting. Assume that there is no knowledge transfer between the tasks and there should be no interference (positive or destructive) when learning one task after the other. Let  (${\bf{X}}_1, y_1$) denote an instance from task 1 and (${\bf{X}}_2$, $y_2$) from task 2. Usually, there are some common tokens (e.g., special tokens) shared across tasks; assume there are  $k$ such tokens.
%. So lets further assume that there are some $k$ such common tokens in these instances. The  

%, for which ${\bf{X}}_1$ and ${\bf{X}}_2$ contain $k$ correlated embeddings. The embeddings corresponding to all other tokens in ${\bf{X}}_1$ and ${\bf{X}}_2$ are assumed to be orthogonal to each other.

%corresponding to those common tokens, while all other embeddings from ${\bf{X}}_1$ are orthogonal to those from ${\bf{X}}_2$.

%Consider the data (${\bf{X}}_1, y_1$) and  (${\bf{X}}_2$, $y_2$) from two orthogonal tasks\nb{what do we mean by orthogonal tasks? that they are unrelated to each other? then just say unrelated tasks?}: Task 1 and Task 2, where ${\bf{X}}_1 \in \mathbb{R}^{n_1 \times d}$ and ${\bf{X}}_2  \in \mathbb{R}^{n_2 \times d}$. Assume there is no knowledge transfer between Tasks 1 and 2, and there should not be interference when learning across tasks. Since there are usually common tokens (e.g., special tokens) shared across tasks, we assume ${\bf{X}}_1$ and ${\bf{X}}_2$ contain $k$ correlated embeddings from those common tokens while all other embeddings from ${\bf{X}}_1$ are orthogonal to those from ${\bf{X}}_2$. Based on Section \ref{sec:single_task_sink}, we assume the correlated tokens are sink tokens.   

%\paragraph{Model.} 
We consider a model consisting of two single-head self-attention layers.  
%The first self-attention layer produces representations for all tokens in the input, which get combined by the second self-attention layer into a single output representation for a prediction token (e.g., \texttt{[CLS]} representation), which is then used for the target task prediction. We consider a regression problem (generalizable to classification), where the prediction for the task $i$ is given by:
\begin{align}
    \hat{y}_i = {\bf{b}}_i^T({\bf{A}}_i{\bf{X}}_i{\bf{W}}){\bf{v}}_i, \nonumber
\end{align}
where ${\bf{X}}_i$ is the input token embeddings, ${\bf{A}}_i \in \mathbb{R}^{n_i \times n_i}$ is the attention matrix generated by the self-attention mechanism, ${\bf{b}}_i \in \mathbb{R}^{n_i}$ contains the attention scores for the prediction token. ${\bf{W}} \in \mathbb{R}^{d \times d}$ is the weight matrix for the attention layer. ${\bf{v}}_i \in \mathbb{R}^{d \times 1}$ is the predictor that maps the $d$-dimensional representation to the output value. 

We now model the attention matrix as ${\bf A}_i = a {\bf 1}$ where $a\in \mathbb R^{n_i}$ has $k$ large magnitude values, corresponding to the $k$ common tokens, and other values are all very close to 0. Then, we may view ${\bf A}_i$ as the adjacency matrix of a directed graph for which the nodes corresponding to common tokens have very high out-degree (e.g. many edges pointing out). 

Now,   even though ${\bf X}_i$ may contain diverse embeddings, almost uniformly distributed across a  high dimensional manifold space, ${\bf A}_i$ will collapse the final embeddings $\hat y_i$ to a low-dimensional space of at most dimension $k$. 
The problem is further exacerbated in fine-tuning, when back propagation learns $\bf W$ and reinforces ${\bf A}_i$; notably, 
\[
\Delta {\bf W} = {\bf X}_i^T  {\bf A}_i^T {\bf b}_i\Delta \hat y_i {\bf v}_i^T, \qquad
\Delta {{\bf  A}_i} =   {\bf b}_i\Delta \hat y_i   {\bf v}_i^T {\bf W}^T {\bf X}_i^T 
\]
which themselves  are at most rank $k$. Over several gradient steps, this will  reduce the rank of both matrices, exacerbating this issue.

%The loss function is:


%For simplicity, we sort each ${\bf{X}}_i$ and ${\bf{A}}_i$ to make the $k$ correlated tokens have index $\{1, ... , k\}$ and others have index $\{(k+1), ..., n_i\}$. 

%However, for text data, there are usually tokens shared across tasks but neutral to task predictions. For example, special tokens like \texttt{[SEP]}; punctuations like `,' and `.'; connecting tokens like `the'; etc. If all correlated tokens\nb{What do you mean by correlated tokens here? Tokens that are shared across tasks?} are neutral tokens, the task-specific information is related to other (orthogonal) tokens in ${\bf{X}}_1$ and ${\bf{X}}_2$. Then there can be two cases: (1). the model pays no attention to correlated tokens and thus the learning on two tasks should not have interference; (2). The model uses neutral tokens to connect other tokens and thus there should only be (limited) task-general interference. 

\paragraph{Claim.} \textit{
The interference between Task 1 and 2 largely depends on the outer degrees of sink tokens and the deviation of all tokens' attention on sink tokens. }

Consider the loss function
$ L(\hat{y}_i, y_i) = \mathbb{E}[\frac{1}{2}(\hat{y}_i - {y}_i)^2]. $
We calculate the interference on the shared parameter $\bf{W}$ by applying Equation~\ref{eqn:cross-task-interference} to the model above:
\begin{align}
    I({\bf{W}}) = (\hat{y}_1 - {y}_1)(\hat{y}_2 - {y}_2)({\bf{B}}_1^T{\bf{B}}_2)({\bf{v}}^T_1{\bf{v}}_2), \label{eqn:interference}
\end{align}
where ${\bf{B}}_i = ({\bf{b}}_i^T{\bf{A}}_i{\bf{X}}_i)^T$ is the representation after attention in Task $i$. When both training losses are not 0 (which is the usual case in CL), the interference depends on the correlation between predictors (${\bf{v}}^T_1{\bf{v}}_2$) and representations (${\bf{B}}_1^T{\bf{B}}_2$). Here we further discuss the correlation ${\bf{B}}_1^T{\bf{B}}_2$.

When the $k$ correlated tokens are sink tokens, we write the $i$-th token's attention on the $j$-th $(j \le k)$ token as ${\bf{A}}_1^{(ij)} = d_1^j + \Delta_1^{(ij)}$   where ${\bf{A}}_1^{(ij)}$ is the $ij$-th element of attention matrix ${\bf{A}}_1$, $d_1^j$ is the average outer degree for the $j$-th token, and $\Delta_1^{(ij)}$ is the deviation between ${\bf{A}}_1^{(ij)}$ and $d_1^j$. Then we have 
\begin{align}
    {\bf{B}}_1     &= \underbrace{\sum\nolimits_{i=1}^{n_1}\sum\nolimits_{j = k+1}^{n_1}{\bf{b}}_1^{i} {\bf{A}}_1^{(ij)}{\bf{X}}_1^{(j \cdot)}}_{\blue{s'_1}:\text{non-sink representations}} + \underbrace{\sum\nolimits_{j = 1}^{k}d_1^{j}{\bf{X}}_1^{(j \cdot)}}_{\red{s_1}: \text{sink representations}} + \underbrace{\sum\nolimits_{i=1}^{n_1}\sum\nolimits_{j = 1}^{k}{\bf{b}}_1^{i} {\Delta}_1^{(ij)}{\bf{X}}_1^{(j \cdot)}}_{{\delta_1}:\text{deviations}}. \label{eqn:single_gradient}
\end{align}

Similarly, we have the non-sink and sink representations $\blue{s'_2}$, $\red{s_2}$ and ${\delta_2}$ for ${\bf{B}}_2$. 

Based on the assumption that non-sink tokens from two tasks are orthogonal, ${s'_1}^T{s'_2} = 0$. Then ${\bf{B}}_1^T{\bf{B}}_2$ depends largely on the correlation between sink representations ${s_1}^T{s_2}$ when (1) \textit{$\delta_1$ and $\delta_2$ are small}: the deviation of all tokens' attention on sink tokens is small, i.e. ${\Delta}_1^{(ij)}$ and ${\Delta}_2^{(ij)}$ are small for $j \le k$. (2). \textit{$s'_1$ and $s'_2$ are small}: sink tokens have large outer degrees, which makes ${\bf{A}}_1^{(ij)}$ small when $j > k$. 
%Since sink tokens are common tokens that should be neutral to most other tokens, when calculating ${s'_1}^T{s_2}$ the dot product between the sink and non-sink token embeddings should be small (Fig. \ref{}). 

\red{[ys: Sorry I'm not really able to follow this part. I think there is a notation to explanation imbalance; try to reduce notation and say stuff in words whenever possible. Or, compress to fewer equations. the logic here is not very clear.]}

When the outer degrees of sink tokens are large, the correlation ${s_1}^T{s_2}$ is also large, which can cause high interference between orthogonal Task 1 and 2. Moreover, when ${\bf{s}}_1$ dominates ${\bf{B}}_1$, models may learn Task 1 by changing sink representations ${\bf{s}}_1$ (Fig. \ref{fig:sink_transfer}(b)). This may distort pre-trained features and make the model less generalizable to OOD data \citep{kumar2022finetuning}. 
 \begin{figure}[htbp]
    \centering
    \includegraphics[width = \linewidth]{Figures/sink_token.jpg}
    \caption{The effect of sink tokens in fine-tuning and transfer learning.}
    \label{fig:sink_transfer}
\end{figure}
\subsection{{Transfer vs. Interference}}
Although attention sinks may propagate unexpected interference, they are important for model capacity. As shown in Fig. \ref{fig:sink_transfer}(a), when removing the attention on sink tokens during training, models have a significant performance drop in the in-task evaluation.

In addition, attention sinks on common tokens may benefit tasks that have knowledge transfer between them. In Fig. \ref{fig:sink_transfer}(a), we conduct experiments that use models trained on 3k MNLI data for zero-shot evaluation on SNLI data, which is under the same sentence entailment task but with a different data distribution. Results show that the transfer ability significantly drops after removing the attention on sink tokens during evaluation. We hypothesize the reason is that sink tokens are common across tasks and can easily transfer knowledge learned on them. 

Based on the above, we do not avoid allocating relatively large attention to sink tokens in CL. Instead, we encourage the model to increase the deviation between different tokens' attention on sink tokens, and allocate more attention on the non-sink tokens to reduce the average outer degrees of sink tokens. Details of the model is shown in Section \ref{sec:method}.

%\paragraph{Forward Transfer.}Over-smoothing can accelerate the feature distortion, which makes the model less generalizable to data from different distributions.
%Experiment list:
%\begin{itemize}
    %\item How oversmoothing influence feature distortion? From the gradient perspective of view. Use feature distortion paper instead of proof.
    %\item OOD performance on BERT and RoBERTa (Yahoo-split?)
    %\item The change of over-smoothing when increasing the training epoch. Over-smoothing becomes more severe after fine-tuning (compare pre-training and fine-tuning). Result unstable, not as expected
%\end{itemize}
%\paragraph{Over-smoothing will reduce the richness of features and make it perform inferior in forward transfer (or even spurious correlation?).}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> wrap_page.tex <==
\iffalse
Consider a node representation matrix ${\bf{X}} \in \mathbb{R}^{n \times d}$ of a graph with the adjacency matrix $\hat{\bf{A}} \in \mathbb{R}^{n \times n}$. Feeding them into a graph convolutional layer with residual connections, the output can be written as: 
\begin{align}
    ResGCN({\bf{X}}) &= {\bf{X}} + \text{ReLU}(\hat{\bf{A}}{\bf{XW}}),  \label{eqn:gcn}  \\
    \hat{\bf{A}} &= {\bf{D}}^{-1/2}{\bf{A}}{\bf{D}}^{-1/2} \nonumber 
\end{align}
where ${\bf{D}}^{n \times n}$ is the degree matrix of the adjacency matrix $\hat{\bf{A}}$. 

Eq. (\ref{eqn:self_attn}) and Eq. (\ref{eqn:gcn}) are similar, where the attention matrix $\hat{\bf{A}}_k$ in Eq. (\ref{eqn:self_attn})  is similar to the normalized adjacency matrix $\hat{\bf{A}}$ in Eq. (\ref{eqn:gcn}). Based on this, the over-smoothing phenomenon in GCN may also happen in Transformer-based models (e.g., BERT).
\fi

\iffalse
\paragraph{Definition 1.} Define $\mathcal{M}:=\{{\bf{Y}} \in \mathbb{R}^{n \times d}|{\bf{Y}} = {\bf{vc}}^T, {\bf{c}} \in \mathbb{R}^{d}\}$ as a subspace in $\mathbb{R}^{n \times d}$, where the vector ${\bf{v}} = [1, 1, ..., 1] \in \mathbb{R}^{n}$. $n$ is the number of input tokens in the sentence, $d$ is the dimension of token representations. The distance of any input representation matrix ${\bf{X}} \in \mathbb{R}^{n \times d}$ to the subspace $\mathcal{M}$ is defined as
\begin{align}
    d_\mathcal{M}({\bf{X}}) :=\inf\{||{\bf{X}} - {\bf{Y}}||_F|{\bf{Y}} \in \mathcal{M}\}, \label{eqn:dist_define}
\end{align}
where $||\cdot||_F$ is the Frobenius norm. 

Eq. (\ref{eqn:dist_define}) evaluates an over-smoothing issue where each token representation in ${\bf{X}}$ is close to the same vector ${\bf{c}}$. Eq. (\ref{eqn:dist_define}) has the infimum value when ${\bf{Y}} = {\bf{ee}}^T{\bf{X}}$, where the vector ${\bf{e}} = n^{-\frac{1}{2}}[1, 1, ..., 1] \in \mathbb{R}^{n} $. This shows when over-smoothing happens, all token representations are close to the averaged token representation, which is ${\bf{c}} = \frac{1}{n}\sum_{i=1}^n {\bf{X}}_i$.
\fi
